GraphFL: A Federated Learning Framework for Semi-Supervised Node Classification on Graphs

Graph-based semi-supervised node classification (GraphSSC) has wide applications, ranging from networking and security to data mining and machine learning, etc. However, existing centralized GraphSSC methods are impractical to solve many real-world graph-based problems, as collecting the entire graph and labeling a reasonable number of labels is time-consuming and costly, and data privacy may be also violated. Federated learning (FL) is an emerging learning paradigm that enables collaborative learning among multiple clients, which can mitigate the issue of label scarcity and protect data privacy as well. Therefore, performing GraphSSC under the FL setting is a promising solution to solve real-world graph-based problems. However, existing FL methods 1) perform poorly when data across clients are non-IID, 2) cannot handle data with new label domains, and 3) cannot leverage unlabeled data, while all these issues naturally happen in real-world graph-based problems. To address the above issues, we propose the first FL framework, namely GraphFL, for semi-supervised node classification on graphs. Our framework is motivated by meta-learning methods. Specifically, we propose two GraphFL methods to respectively address the non-IID issue in graph data and handle the tasks with new label domains. Furthermore, we design a self-training method to leverage unlabeled graph data. We adopt representative graph neural networks as GraphSSC methods and evaluate GraphFL on multiple graph datasets. Experimental results demonstrate that GraphFL significantly outperforms the compared FL baseline and GraphFL with self-training can obtain better performance.

==> commands.tex <==
\usepackage{epsf}
%\usepackage{fancyheadings}
\usepackage{graphics}
%\usepackage{graphicx}

%\usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{psfrag}

\usepackage{color}

\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{fdsymbol}
%\usepackage[linesnumbered, ruled, vlined]{algorithm2e}
%\usepackage{ntheorem}

%\usepackage[backend=bibtex,firstinits=true]{biblatex}

%\setlength{\textwidth}{\paperwidth}
%\addtolength{\textwidth}{-6cm}
%\setlength{\textheight}{\paperheight}
%\addtolength{\textheight}{-4cm}
%\addtolength{\textheight}{-1.1\headheight}
%\addtolength{\textheight}{-\headsep}
%\addtolength{\textheight}{-\footskip}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS HERE

%%%%%%%
%\theoremstyle{plain}

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper

%\theoremprework{\begin{minipage}{\textwidth}}
%\theorempostwork{\end{minipage}}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{assumption}{Assumption}
\newtheorem{exmp}{Example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
%\newlength{\widebarargwidth}
%\newlength{\widebarargheight}
%\newlength{\widebarargdepth}
%\DeclareRobustCommand{\widebar}[1]{%
%  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
%  \settoheight{\widebarargheight}{\ensuremath{#1}}%
%  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
%  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
%    \hspace{0.3\widebarargdepth}%
%    \addtolength{\widebarargheight}{0.3ex}%
%    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
%  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
%\makeatletter
%\long\def\@makecaption#1#2{
%        \vskip 0.8ex
%        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
%        \parindent 1.5em  %% How can we use the global value of this???
%        \dimen0=\hsize
%        \advance\dimen0 by -3em
%        \ifdim \wd\@tempboxa >\dimen0
%                \hbox to \hsize{
%                        \parindent 0em
%                        \hfil 
%                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
%                                {\bf #1.} #2
%                                %%\unhbox\@tempboxa
%                                } 
%                        \hfil}
%        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
%        \fi
%        }
%\makeatother

\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\ordertil}{\ensuremath{\widetilde{\order}}}
\newcommand{\w}{\bm{w}}
\newcommand{\al}{\bm{\alpha}}

%% COMMENTING commands

\long\def\comment#1{}

\newcommand{\bm}[1]{\boldsymbol{#1}}
\newcommand{\llVert}{\left\lVert}
\newcommand{\rrVert}{\right\rVert}
\newcommand{\bit}[1]{\boldsymbol{#1}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\mjwcomment}[1]{{\bf{{\red{{MJW --- #1}}}}}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\mycomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\vidyacomment}[1]{{\bf{{\green{{VM --- #1}}}}}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\cmcomment}[1]{{\bf{{\cyan{{CM --- #1}}}}}}

% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

\newcommand{\defn}{:\,=}

%Hamming metric
\newcommand{\dH}{\mathsf{d}_{\mathsf{H}} }

\newcommand{\id}{\mathsf{id}}

\newcommand{\KT}{\mathsf{KT}}

\newcommand{\dimone}{n_1}
\newcommand{\dimtwo}{n_2}
\newcommand{\maxdimonetwo}{\left(\dimone \lor \dimtwo \right)}

\newcommand{\Aone}{{\bf C1} }
\newcommand{\Atwo}{{\bf C2} }

\newcommand{\csst}{\mathbb{C}_{\mathsf{SST}}}
\newcommand{\cdiff}{\mathbb{C}_{\mathsf{DIFF}}}
\newcommand{\Cpara}{\mathbb{C}_{\mathsf{PARA}}}
\newcommand{\Cbiso}{\mathbb{C}_{\mathsf{BISO}}}
\newcommand{\Cns}{\mathbb{C}_{\mathsf{NS}}}
\newcommand{\Cnspi}{M_{\mathsf{NS}, \pi}}
\newcommand{\Mns}{M_{\mathsf{NS}}}
\newcommand{\Cnspihat}{M_{\mathsf{NS}, \pihat}}

\newcommand{\sk}{S_k}
\newcommand{\bl}{\mathsf{bl}}

\newcommand{\bltilde}{\widetilde{\mathsf{bl}}}
\newcommand{\Bl}{\mathsf{B}}
\newcommand{\Rw}{\mathsf{R}}

\newcommand{\tauhat}{\widehat{\tau}}
\newcommand{\Chatt}{\widehat{C}_t}

\newcommand{\rhat}{\widehat{\mathsf{r}}}
\newcommand{\rspace}{\mathsf{r}}

\newcommand{\elts}{\mathsf{s}}
\newcommand{\Ntilde}{\widetilde{N}}

\newcommand{\lambdahat}{\widehat{\lambda}}

\newcommand{\Cmodel}{\mathbb{C}}

\newcommand{\pobs}{p_{\mathsf{obs}}}

\newcommand{\sgn}{\mathsf{sgn}}

\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{fro}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}


% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% Kullback-Leibler
\newcommand{\kull}[2]{\ensuremath{D(#1\; \| \; #2)}}

% Probability
\newcommand{\E}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

% Observations, dimension etc.
\newcommand{\numobs}{\ensuremath{n}}
\newcommand{\usedim}{\ensuremath{d}}

\newcommand{\Comp}{\ensuremath{C}}

\newcommand{\Mrisk}{\ensuremath{\mathcal{M}}}
\newcommand{\Erisk}{\ensuremath{\mathcal{E}}}
\newcommand{\Arisk}{\ensuremath{\mathcal{A}}}

\newcommand{\diam}{\ensuremath{\mathsf{diam}}}
%Numbering
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}

\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\child}{child}
\DeclareMathOperator{\parent}{parent}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{{\sf rank}}
\DeclareMathOperator{\card}{{\sf card}}
\DeclareMathOperator{\range}{{\sf range}}
\DeclareMathOperator{\toeplitz}{toeplitz}


% 
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}

\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}
\newcommand{\Ospace}{\ensuremath{\mathcal{O}}}

\newcommand{\Bupper}{\ensuremath{\overline{B}}}
\newcommand{\Blower}{\ensuremath{\underline{B}}}
% Basic statistics notation
% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimate one
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}

\newcommand{\xhat}{\ensuremath{\widehat{x}}}
\newcommand{\Deltahat}{\ensuremath{\widehat{\Delta}}}

\newcommand{\Deltatilde}{\ensuremath{\widetilde{\Delta}}}
\newcommand{\udiff}{\ensuremath{\mathbb{U}^{{\sf diff}}_m(A)}}
\newcommand{\Xhat}{\ensuremath{\widehat{X}}}
\newcommand{\Yhat}{\ensuremath{\widehat{Y}}}
\newcommand{\Ytilde}{\ensuremath{\widetilde{Y}}}
\newcommand{\Mhat}{\ensuremath{\widehat{M}}}
\newcommand{\Mstar}{\ensuremath{M^*}}
\newcommand{\Mtilde}{\ensuremath{\widetilde{M}}}
\newcommand{\bhat}{\ensuremath{\widehat{b}}}
\newcommand{\Mhatasp}{\ensuremath{\widehat{M}}_{\mathsf{ASP}}}
\newcommand{\ASP}{\ensuremath{\mathsf{ASP}}}

\newcommand{\CRL}{\ensuremath{\mathsf{CRL}}}

\newcommand{\Mhattds}{\ensuremath{\widehat{M}}_{{\sf TDS}}}

\newcommand{\Mhatod}{\ensuremath{\widehat{M}}_{{\sf 1D}}}
\newcommand{\Mhatls}{\ensuremath{\widehat{M}}_{{\sf LS}}}
\newcommand{\Mhatpermr}{\ensuremath{\widehat{M}}_{{\sf permr}}}

\newcommand{\BAP}{\ensuremath{\mathsf{BAP}}}
\newcommand{\agg}{\ensuremath{\mathsf{Agg}}}
\newcommand{\Mhatbap}{\ensuremath{\widehat{M}}_{\mathsf{BAP}}}

\newcommand{\Btilde}{\ensuremath{\widetilde{B}}}

\newcommand{\xhatml}{\ensuremath{\widehat{x}_{{\sf ML}}}}
\newcommand{\Xhatml}{\ensuremath{\widehat{X}_{{\sf ML}}}}
% Estimate two
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

\newcommand{\gt}{\ensuremath{\widetilde{g}}}

\newcommand{\yvec}{\ensuremath{y}}
\newcommand{\Xmat}{\ensuremath{X}}

\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}


%Problem-specific notation
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
\newcommand{\real}{\ensuremath{\mathbb{R}}}

\newcommand{\Pihat}{\ensuremath{\widehat{\Pi}}}
\newcommand{\pihat}{\ensuremath{\widehat{\pi}}}
\newcommand{\pihatborda}{\ensuremath{\widehat{\pi}_{\sf bor}}}
\newcommand{\pihatpre}{\ensuremath{\widehat{\pi}_{\sf pre}}}
%\newcommand{\pihatref}{\ensuremath{\widehat{\pi}_{\sf ref}}}
\newcommand{\pihattds}{\ensuremath{\widehat{\pi}_{\sf tds}}}
\newcommand{\pihatoned}{\ensuremath{\widehat{\pi}_{{\sf 1D}}}}
\newcommand{\pihatftds}{\ensuremath{\widehat{\pi}_{{\sf tds}}}}
\newcommand{\sigmahat}{\ensuremath{\widehat{\sigma}}}
\newcommand{\Sigmahat}{\ensuremath{\widehat{\Sigma}}}
\newcommand{\sigmahatborda}{\ensuremath{\widehat{\sigma}_{\sf bor}}}
%\newcommand{\sigmahatref}{\ensuremath{\widehat{\sigma}_{\sf ref}}}
\newcommand{\sigmahattds}{\ensuremath{\widehat{\sigma}_{\sf tds}}}
\newcommand{\sigmahatftds}{\ensuremath{\widehat{\sigma}_{\sf tds}}}
\newcommand{\sigmahatpre}{\ensuremath{\widehat{\sigma}_{\sf pre}}}

\newcommand{\pihatasp}{\ensuremath{\widehat{\pi}_{\mathsf{ASP}}}}
\newcommand{\Pihatml}{\ensuremath{\widehat{\Pi}_{{\sf ML}}}}
\newcommand{\Pitil}{\ensuremath{\widetilde{\Pi}}}

\newcommand{\Projpi}{\ensuremath{P_{\Pi}}}
\newcommand{\Projorthpi}{\ensuremath{P_{\Pi}^{\perp}}}
\newcommand{\Projorthpistar}{\ensuremath{P_{\Pi^*}^{\perp}}}

\newcommand{\hballpi}{\ensuremath{\mathbb{B}^{\sf H}_\Pi}}
\newcommand{\hballpistar}{\ensuremath{\mathbb{B}_{\sf H}}}
%\newcommand{\hballpistar}{\ensuremath{\mathcal{P}_n}}
\newcommand{\SNR}{\ensuremath{\frac{\|x^*\|_2^2}{\sigma^2}}}
\newcommand{\col}{\ensuremath{{\sf col}}}
\newcommand{\row}{\ensuremath{{\sf row}}}
\newcommand{\Pn}{\ensuremath{\mathcal{P}_n}}

\newcommand{\EE}{\ensuremath{\mathbb{E}}}
%changed to probability of error
\newcommand{\Rpihat}{\ensuremath{\Pr\{ \Pihat \neq \Pi^* \} }}

\newcommand{\Rpihatml}{\ensuremath{\Pr\{ \Pihatml \neq \Pi^* \}}}
\newcommand{\BigO}{\ensuremath{\mathcal{O}}}


\newcommand{\numitems}{\ensuremath{n}}

% commands that CM changed/introduced
\newcommand{\symgp}{\mathfrak{S}}
\newcommand{\vars}{\zeta}
\newcommand{\maxvarone}{(\vars^2 \lor 1)}
\newcommand{\varplusone}{(\vars + 1)}
\newcommand{\allones}{\mathbf{e}}
\newcommand{\bfone}{\mathbf{1}}
\DeclareMathOperator{\trace}{\mathsf{tr}}
\DeclareMathOperator{\Poi}{\mathsf{Poi}}
\DeclareMathOperator{\var}{\mathsf{var}}
\DeclarePairedDelimiter\tv{\mathsf{tv}(}{)}

%\newcommand{\Cperm}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{r},\mathsf{c}}}
\newcommand{\Cperm}{\mathbb{C}_{\mathsf{Perm}}}
%\newcommand{\Cpermr}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{r}}}
%\newcommand{\Cpermc}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{c}}}
\newcommand{\Cskew}{\mathbb{C}_{\mathsf{skew}}}

\newcommand{\tds}{{\sf TDS}}

\newcommand{\Ypoi}{Y_{\sf Poi}}
%\newcommand{\Ysortcol}{Y_{\sf sortcol}}
%\newcommand{\Ysortrow}{Y_{\sf sortrow}}

\newcommand{\BL}{\mathsf{BL}}

\newcommand{\Mps}{M_{\pi, \sigma}}
\newcommand{\Dps}{\Delta_{\pi, \sigma}}
\newcommand{\Cdiffps}{\cdiff(\pi, \sigma)}
\newcommand{\Zps}{Z_{\pi, \sigma}}
\newcommand{\Ztil}{\Zps}
\newcommand{\At}{\mathcal{A}_t}
\newcommand{\Wtil}{\widetilde{W}}
\newcommand{\cE}{\mathcal{E}}

\newcommand{\bllarge}{\mathsf{BL}^{\mathbb{L}}}
\newcommand{\blsmall}{\mathsf{BL}^{\mathbb{S}}}
%\newcommand{\blunion}{\cup \mathsf{bl}}
%\newcommand{\bllargeunion}{\cup \bllarge}
%\newcommand{\blsmallunion}{\cup \blsmall}
\newcommand{\blone}{\BL^{(1)}}
\newcommand{\bltwo}{\BL^{(2)}}
%\newcommand{\blthree}{\BL^{(3)}}
\newcommand{\blt}{\BL^{(t)}}
%\newcommand{\bltp}{\BL^{(t')}}

\newcommand{\blocksize}{\dimtwo \sqrt{\frac{\dimone}{N} \log (\dimone \dimtwo) }}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

